GSEdit: Efficient Text-Guided Editing of 3D Objects via Gaussian Splatting

We present GSEdit, a pipeline for text-guided 3D object editing based on Gaussian Splatting models. Our method enables the editing of the style and appearance of 3D objects without altering their main details, all in a matter of minutes on consumer hardware. We tackle the problem by leveraging Gaussian splatting to represent 3D scenes, and we optimize the model while progressively varying the image supervision by means of a pretrained image-based diffusion model. The input object may be given as a 3D triangular mesh, or directly provided as Gaussians from a generative model such as DreamGaussian. GSEdit ensures consistency across different viewpoints, maintaining the integrity of the original object's information. Compared to previously proposed methods relying on NeRF-like MLP models, GSEdit stands out for its efficiency, making 3D editing tasks much faster. Our editing process is refined via the application of the SDS loss, ensuring that our edits are both precise and accurate. Our comprehensive evaluation demonstrates that GSEdit effectively alters object shape and appearance following the given textual instructions while preserving their coherence and detail.

==> 01b-relwork/main.tex <==

\noindent
\daniele{Below is a draft for the related work paragraphs. It might be a good idea to include DreamGaussian in the related work, but we need to fit it into one of the paragraphs above or think of a new one.}
\paragraph*{Inverse rendering} \daniele{Nerf, gaussian splatting, small references to various lines of research in the field\\
\begin{itemize}
    \item NeRF
    \item MipNeRF
    \item zipNeRF
    \item instantNeRF
    \item Gaussian Splatting
\end{itemize}
}
\paragraph*{3D object editing} \daniele{Here we can discuss style transfer, texture synthesis, and I'm sure there's a ton of recent works I haven't kept track of that are worth citing. Clearly, instruct-nerf2nerf.\\
\begin{itemize}
    \item NeRF-Art
    \item InstructN2N
    \item VoxE
    \item LatentEditor?
    \item GaussianEditor?
\end{itemize}
}

\paragraph*{Text-to-image generation} \daniele{A bunch of stuff on diffusion models, IP2P, ...\\
\begin{itemize}
    \item Instrut-Pix2Pix
    \item EmuEdit?
    \item MagicBrush
    \item Imagic
    \item DiffEdit
\end{itemize}
}

\noindent
\daniele{These paragraphs below need to be reorganized according to the structure above}


\paragraph*{Inverse rendering} Recent research in inverse rendering and multi-view synthesis led to significant progress in a variety of complex problems in 3D vision/graphics. Mildenhall \etal~\cite{mildenhall2020nerf} were the first to propose the idea of optimizing volumetric color/density functions encoded by deep neural networks via differentiable volumetric rendering. This provided a novel, general framework to handle geometry in an implicit fashion, thus bypassing all issues derived from explicit structures such as triangle meshes. Over the years, the original contribution has been studied and improved over several aspects. \daniele{List sub-research areas for NeRF, end with Gaussian Splatting}



\paragraph*{3D object editing}
% One of the most important work on 3D scene editing is Instruct-NeRF2NeRF \cite{haque2023instructnerf2nerf} (\textbf{IN2N}). As the name may suggest, it is a NeRF-based approach that uses InstructPix2Pix \cite{brooks2023instructpix2pix} (\textbf{IP2P}) to change the details and appearance of the NeRF scene. These methods yield good results; however, they take a lot of time to apply changes ($\sim 2h$).

\paragraph*{Text-driven Image editing?}
%https://arxiv.org/pdf/2312.11396.pdf
% In text-driven image editing, the fusion of language and visual content has progressed significantly, with models like CLIP and various diffusion approaches enabling more intuitive and detailed manipulations based on textual descriptions. This integration facilitates a more user-centric editing process, accommodating abstract concepts or specific styles through language.

\paragraph*{3D Scene Reconstruction}
% All these methods are based on NeRF \cite{mildenhall2020nerf}, or one of his variants like Mip-NeRF \cite{barron2021mipnerf}, making the process of 3D generation slow. An important breakthrough in 3D scene reconstruction from images is the Gaussian Splatting \cite{kerbl20233d}. This novel method is tens of times faster than the previous methods,
% and still delivers high quality results. 

% \paragraph*{Last works on prompt to 3D}
% The two main papers that currently exploit this novel technique for prompt to 3D generation are GSGen \cite{chen2023textto3d} and DreamGaussian \cite{tang2023dreamgaussian} (\textbf{DG}). The former introduced a compactness-based densification and a geometry optimization stage, while the latter introduced an efficient algorithm to con

